Self-supervised Temporal Discriminative Learning for Video Representation Learning

Temporal cues in videos provide important information for recognizing actions accurately. However, temporal-discriminative features can hardly be extracted without using an annotated large-scale video action dataset for training. This paper proposes a novel Video-based Temporal-Discriminative Learning (VTDL) framework in self-supervised manner. Without labelled data for network pretraining, temporal triplet is generated for each anchor video by using segment of the same or different time interval so as to enhance the capacity for temporal feature representation. Measuring temporal information by time derivative, Temporal Consistent Augmentation (TCA) is designed to ensure that the time derivative (in any order) of the augmented positive is invariant except for a scaling constant. Finally, temporal-discriminative features are learnt by minimizing the distance between each anchor and its augmented positive, while the distance between each anchor and its augmented negative as well as other videos saved in the memory bank is maximized to enrich the representation diversity. In the downstream action recognition task, the proposed method significantly outperforms existing related works. Surprisingly, the proposed self-supervised approach is better than fully-supervised methods on UCF101 and HMDB51 when a small-scale video dataset (with only thousands of videos) is used for pre-training. The code has been made publicly available on https://github.com/FingerRec/Self-Supervised-Temporal-Discriminative-Representation-Learning-for-Video-Action-Recognition.

==> figures/1-Augment_Background.tex <==
\begin{figure}
  \centering
  \includegraphics[width=1\linewidth]{figs/augment_background.png}
  \caption{Our intuition: The action keep \textit{temporal consistent} with static background replacement. 
  Human can still tell this action is \textit{tai chi} even though the appearance difference between the two videos is huge.}
  \label{fig:bk_replace}
\end{figure}


==> figures/1-Temporal_Background.tex <==
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figs/temporal_background.png}
  \caption{The motivation of our proposed Temporal Consistent Augmentation(TCA). Some actions exist significant correlation over static background or object. e.g. recognize ``swimming'' by ``water'', ``ride horse'' by ``horse''. But mainly focus on spatial content may caused that the complex action like ``ride horse in water'' will be easily confused with ''swimming'' by ''water'' instead of temporal cues.}
  \label{fig:temporal_background}
\end{figure}


==> figures/3-1-VideoTriplet.tex <==
\begin{figure}
  \centering
  \includegraphics[width=.8\linewidth]{figs/video_triplet.png}
  \caption{ Illustration for a training batch with two examples. Blue edges and red edges represent similar and dissimilar examples respectively. 
  Our method explicitly generate triplet for each sample and takes into account all pairs between \textit{anchors}.}
  \label{fig:video_triplet_cmp}
\end{figure}


==> figures/3-3-Triplet_single.tex <==
\begin{figure}
  \centering
  \includegraphics[width=.8\linewidth]{figs/triplet_single.png}
  \caption{We visualize one example of Triplet. The optical flow grad is get by \cite{meinhardt2013horn}}.
  \label{fig:triplet_single}
\end{figure}


==> figures/4-5-class.tex <==
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figs/hmdb51_relative_performance.png}
  \caption{The relative performance of VTDL vs. Scratch on HMDB51. We select top-5 largest and lowest class. VTDL outperforms the Scratch when actions are dynamic.}
  \label{fig:class}
\end{figure}


==> figures/4-5-heatmap.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=\linewidth]{figs/heatmap_visualization.png}
  \caption{The heatmap visualization.}
  \label{fig:heatmap}
\end{figure*}


==> figures/4-5-tsne.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=\linewidth]{figs/t-sne.png}
  \caption{The heatmap visualization.}
  \label{fig:tsne}
\end{figure*}


==> figures/ba_tca.tex <==
\begin{figure*}[b]
  \centering
  \includegraphics[width=\linewidth]{figs/supplementary_ba_tca.png}
  \caption{Visualization of the generated \textit{anchor} and \textit{positive} (with BA and TCA).}
  \label{fig:ba_tca_visualize}
\end{figure*}

==> sections/acknowlegment.tex <==

\section{Acknowledgments}

Identification of funding sources and other support, and thanks to
individuals and groups that assisted in the research and the
preparation of the work should be included in an acknowledgment
section, which is placed just before the reference section in your
document.

This section has a special environment:
\begin{verbatim}
  \begin{acks}
  ...
  \end{acks}
\end{verbatim}
so that the information contained therein can be more easily collected
during the article metadata extraction phase, and to ensure
consistency in the spelling of the section heading.

Authors should not prepare this section as a numbered or unnumbered {\verb|\section|}; please use the ``{\verb|acks|}'' environment.



==> sections/bk.tex <==
========================0=========================
Self-supervised learning has achieved great success for visual understanding of still images. 
However, due to the widely-used video datasets have serious implicit bias and a limited number of samples, the advantage over traditional methods is not so evident in video understanding.
This paper aims to discover the principles to design effective unsupervised techniques for semantic understanding in videos and learn these models given limited and bias unlabeled training samples. 
Our first contribution is Temporal Consistent Augmentation (TCA), a novel data augmentation method for video understanding, which is based on the idea of background replacement. 
The other contribution is the Video-based Triplet Learning (VTL) framework, which generates video triplets and the target is to let the temporal-similarity pairs closer than temporal-dissimilarity pairs in the learned embedding space. 
It combines (a) generate triplet for each sample and (b) video-based triplet learning. The resulting embedding network can be transferred to down-stream video understanding tasks. 
In action recognition, our approach significantly outperforms previous state-of-the-art related work even better than fully-supervised pre-train when the amount of hand-crafted label data in thousands level. Source code will be made publicly available.



===============================1===========================
% \section{Introduction}

% Video action recognition is an important problem which benefits high-level perception tasks including video caption \cite{guadarrama2013youtube2text} and video action detection \cite{zhu2017flow}. 
% However, learning visual representations generally requires a large number of labeled training examples.
% This is especially true for video, because video is a higher-dimensional input than images, and video CNN has more parameters to learn than 2D CNN.
% Simultaneously, videos are more expensive to collect and annotate than images, as they require additional, and often ambiguous, temporal annotations.
% This calls for methods that can be trained on any size datasets with no supervision.

% Self-supervised learning (SSL), especially contrastive learning \cite{hadsell2006dimensionality}, has been widely studied in the Machine Learning community and achieve highly successful in image-based tasks like image classification, object detection \cite{wang2019self,he2019momentum}, and natural language processing \cite{devlin2018bert}.
% The target of SSL is to Pre-training the base models with proxy task.
% A key reason for their success is that they can be applied on any specific domain and the large size of image and text dataset.

% However, in video-based action recognition, supervised pre-training is still dominant \cite{carreira2017quo, wang2018non}, where self-supervised methods generally lag behind.
% Action is defined as:
% \begin{quoting}[font=itshape, begintext={``}, endtext={''---P. Turaga\cite{turaga2008machine}}]
% simple motion patterns usually executed by a single person and typically lasting for a very short duration (order of tens of seconds).
% \end{quoting}
% which means incorporate temporal structure, which make the task more challenge than image.

% % In this paper, we present a new, principled method for unsupervised learning of video representations from unlabeled video data.
% % It is based on the observation that is often sufficient to learn good feature representations.
% % Importantly, we demonstrate that such combination could be found without per-class or per-video labeling by instead matching.

% In our view, the application of self-supervised learning in video understanding is impeded by two major obstacles.
% \textit{First}, training deep CNNs requires a large volume of training samples to achieve optimal performance.
% However, due to the difficulty in data collection and annotation, publicly available video understanding datasets for self-supervised learning remain limited (e.g. UCF101 \cite{soomro2012ucf101}, HMDB51 \cite{kuehne2013hmdb51}), in both size and diversity.
% Consequently, large 3D CNNS, which have attained remarkable success in action recognition, are confronted with high risk of over-fitting.
% \textit{Second}, temporal structure plays an important role in understanding the dynamic in videos. 
% To learn visual temporal.
% These video datasets exist huge implicit bias over scene and object structure \cite{girdhar2019cater,shao2020finegym}, that is, a large amount of samples can be recognized via object or background. e.g., recognize ``swimming'' via water. 
% In this way, the temporal modeling become less important and the network go back to static image representation.
% % However, this serious problem is less studied .
% However, mainstream self-supervised methods may focus on appearance or trivial solution, thus lacking the capacity to incorporate temporal structure.

% These challenges motivate us to study two problems:
% 1) how to learn the CNN models given limited training samples.
% 2) how to design an effective and efficient video self-supervised framework for learning video representation that is able to prevent trivial solution. %object bias
% In particular, we build our method on top of the successful 3D CNN architecture which good at tackling the temporal modeling mentioned above.
% In terms of limited samples, two key observations are that the consecutive frames are highly redundant especially in background and exist dataset have significantlly object implicit bias.
% Motivated by these observations, we propose two novel data augmentation techniques Intra-video Mixup and Inter-Video mixup for video understanding.
% These methods introducing natural global noise from the same or different video frame-wise, which keep the semantic but large difference in appearance.
% %Temporal Consistent Augmentation


% Moreover, we develop a video-level framework, called Video-based Triplet Learning (VTL).
% VTL is a mechanism for building dynamic triplet based dictionaries for contrastive learning, and can be used with various pretext tasks. 
% As our main purpose is to pre-train representations that can be transfered to downstream tasks by fine-tuning. 
% We shown that in downsteam action recognition VTL can surpass its Imagenet supervised counterpart, even surpass fully-supervised in thousands level dataset. 
% These results show that VTL largely close the gap between unsupervised and supervised representation learning, and can serve as an alternative to ImageNet supervised pre-training in video action recognition.

% The main contributions are:
% \begin{itemize}
%     \item We propose hard-triplet with novel data augmentation.
%     \item A novel self-supervised framework that work with any backbones is proposed and achieve significantlly improvement in UCF101 and HMDB51.
%     \item We also visualize the our learned models trying to provide some insights for future video understanding research.
% \end{itemize}

% %contribution: 1. generate triplet with data augmentation
% %2. propose a novel triplet loss

================================3.1=========================
% \subsection{Background}
% \label{sec:cl}

% %instance-lebel discrimination.
% %Contrastive learning is a way of building a discrete dictionary on high-dimensional continuous inputs such as images.
% %Need a memory bank.
% %Based on MoCo \cite{he2019momentum}.
% %The contrastive loss serves as an unsupervised objective function.
% %In general, the query representation is $q=f_q(x^q)$ where $f_q$ is an encoder network and $x_q$ is a query sample. 
% %Formally, suppose we mapping a random sample into the queue $q$. 
% %where $\tau$ is a temperature hyper-parameter which control the importance of each item.

% Contrastive learning \cite{hadsell2006dimensionality} learn a good embedding which should keep map visually similar samples closer to each other. 
% Common practice \cite{wu2018unsupervised, he2019momentum, chen2020simple} treat each sample instance as a distinct class of its own and train a classifier to distinguish between individual instance classes.
% Specifically, for all samples in $D$, their high-level representation is $q_1,...,q_n$ are $q_i=f_\theta(q_i)$. 
% For each sample, the positive keys are a same sample with different data augmentation or view (denoted as key $k_i^{+}$) and all the others samples are record as key $k_i^{-}$.
% Contrastive loss is a function whose value is low when $q$ is similar to its positive key $k^{+}$ and dissimilar to $k^-$ (considered negative keys for $q$).
% With similarity measured by $d$, a form of a contrastive loss function, is:
% \begin{equation}
%     \label{eq:1}
%     L = \sum_{i=1}^{n} - log \frac{d(q_i, k_i^+) }{d(q_i, k_i^{+}) + d(q_i, k_i^{-})}
% \end{equation}
% From above equation, $k^-$ must be saved in a memory bank and available at any time during training.

% However, as the number of $n$ become very large, computing the similarity to all the instances in the training set is very time consuming. 
% In addition, save the queues of all samples in a memory bank is memory consumption.
% To tackle these problems, \cite{wu2018unsupervised} use NCE to approximate the memory bank and \cite{ye2019unsupervised} compute contrastive loss in a mini-batch.
% Recently proposed MoCo \cite{he2019momentum}, which is considered in this paper, maintaining the memory bank as a \textit{queue} of data samples, which progressively replaced the samples in the queue. 
% During training, the new features are enqueued to the queue and the oldest in the queue is removed for each mini batch.
% MoCo adopt two networks $\theta_q$ and $\theta_k$ for query $q$ and key $k$, but only query network is update by back propagation and the key network is update moment.
% Formally, denoting the parameters of $f_k$ as $\theta_{k}$ and those of $f_q$ as $\theta_{q}$, in each iteration update $\theta_{k}$ by:
% \begin{equation}
%     \theta_{k} = m \theta_{k} + (1-m) \theta_{q}
% \end{equation}
% here $m$ is a momentum coefficient.


% Contrastive loss is a function whose value is low when $x$ is similar to its augmentation data $\hat{x}_i$ and dissimilar to the other samples.

% \subsubsection{Triplet Learning} \cite{schroff2015facenet} directly optimize the embedding itself via generate all possible triplets. The triplet loss minimizes the distance between an \textit{anchor} and a \textit{positive} (same identity), and maximizes the distance between a \textit{anchor} and a \textit{negative} (different identity). Instead of requiring multiple instance, we generate triplet with single video.

%In this subsection, we briefly review recent works on discriminatively training networks to learn semantic embeddings.

% \begin{equation}
%     x_i^{(j)} = \alpha \times x_i^{(j)} + (1 - \alpha) \times x_i^{(k)}, i=1,\cdot,T
% \end{equation}
% where $k \in [1,T]$ and $\alpha$ is uniform sampling from $[0,0.5]$.
% The inter-video mixup select one frame from another video and interpolate frame-wise, formally
% \begin{equation}
%     x_i^{(j)} = \alpha \times x_i^{(j)} + (1 - \alpha) \times x_l^{(k)}, i=1,\cdot,T
% \end{equation}



% \subsubsection{Video-based Triplet Loss}
% We illustrate the generation of our triplet in Figure \ref{fig:triplet}. 
% For each video, we select one spatio-temporal clip at random location, named as \textit{anchor}. 
% Then, we crop the video in the same temporal location but different spatial, called as \textit{positive}.
% On the contrary, \textit{Negative} is sampling from different temporal localization but no requirement for spatial location.
% The begin index of \textit{anchor} and \textit{negative} at least vary $\tau$. Formally,
% \begin{equation}
%     |b_a - b_n| > \tau
% \end{equation}
% where $b_a$ and $b_n$ for begin index of \textit{anchor} and \textit{negative}.
% In order to improve the diversity of each sample and prevent overfitting, we adopt Basic Augmentation for generated triplet.
% Basic Augmentation of this type of transformation such actions as scale, occlusion, lighting, rotation or any combination of these (\cref{sec:id}).
% To overcome object bias and make the distinguish task more hard, we propose novel Framewise Global Noise, which introduce strong interference noise framewise and consequently show large variant in background.
% A form of a triplet contrastive loss function, is:
% \begin{equation}
%     \label{eq:2}
%     L = \sum_{i=1}^{n} - log \frac{d(v_i^a, v_i^p) }{d(v_i^a, v_i^p) + d(v_i^a, v_i^n) + \sum_{j \neq i}^{} d(v_i^a, v_j^a)}
% \end{equation}
% \subsection{Hard Triplet Generating.}
% % \textbf{Framewise Global Noise.}
% \textbf{Hard Positive.}
% \textbf{Hard Negative.}
% We begin with define interpolation as: given a \textit{fixed} frame and an input video clip, interplate with all the frames in video clip with probability $\alpha$ framewise. Here $\alpha$ is uniform sampling from $[0,0.5]$.
% And in this work we propose two novel data augmentation methods that introduces global noise: Intra-Sample and Inter-Sample interpolation. 
% While the former select \textit{fixed} frame from same video and the latter select from different video.
% Further, taking inspiration from Cutup \cite{devlin2018bert}, we random select one region and cut it from each frame in the same location and called as Video Cutup.
% Notice all these techniques introducing same global noise framewise and show large variance in appearance but keep semantic consistency for random video.

% \subsubsection{Motivation.}
% Our motivations behind this setup are as follows:
% \emph{i}.
% Considering \textit{anchor} and \textit{positive} pairs, the core idea is that two spatio-temporal clips coming from the same time but different spatial location share similar semantic but large difference in pixel.
% This correspondence encourages learning invariance to Basic Augmentation, Framewise Global Noise and different spatial viewpoint, since the \textit{positive} and \textit{anchor} frames show the same action with variations along these factors.
% \emph{ii}.
% Since temporal neighbors are visually similar and augmented with same Weak Augmentation, the only way to tell \textit{anchor} and \textit{negative} apart is to model the motion of objects or humans.

% \subsubsection{Predict Pseudo Label.}
% Considering the similarity of two videos with same action, especially in same scene.
% while Contrastive Learning act as instance discrimination task, the learned network may focus on trivial solution.
% We believe that generate pseudo label and retrain the network can smooth the feature space and weaken the underlying pre-training objective-specific bias.
% For this purpose, we use the learned model with contrastive learning to extract features from each datapoint belonging to $D$.
% Next, we cluster these features using k-means into $K$ groups and treat these cluster assignments as the new categorical labels for $D$.
% Finally, we train this network that minimizes a cross-entropy objective under the supervision of these generated pseudo labels.


% \label{sec:id}
% In this section we first introduce the basic data augmentation in this paper.
% Then, we describe the base network and projection head.
% Finally, the pseudo label prediction detials are given.


% \textbf{Pseudo Label Prediction}
% We extract features from the global spatial average pooling layer from the backbone, and then reshape as an vector.
% For clustering, features are PCA-reduced to 256 dimensions, and $l_2$ normalized.

% For the predict pseudo label tasks, we followed by a fully connect layer after global average pooling layer, the final output dimension is $K$. 

% Constrastive learning is a way of building a discrete dictionary on high-dimensional continuous inputs. 
% Our hypothesis is that good features can be learned by construct more hard distinguished samples, while the encoder for the keys is kept as consistent as possible despite its evolution.
% Further, the network only optimize by contrastive loss may focus on trivial solution rather than general representation. 
% We believe that triplet contrastive learning followed by clustering and prediction can smooth the feature space.
% Based on these motivations, we propose progressive triplet contrastive (PTC) learning framework as described next.
%To better take advantage of the representations, we iteratevely train the models until convergence.

==> sections/introduction_bk_5_10.tex <==

\section{Introduction}

% ======================1.image recognition vs. action recognition===============
Image recognition has achieve remarkable progress recently years \cite{szegedy2017inception}, particularly the development of many new CNNs \cite{he2016deep} and large-scale benchmarks. 
However, video-based action recognition is lag behind.
Compared with image recognition, the major obstacles lie in that: 
The definition of action is as noted by Turage et al. \cite{turaga2008machine}, ``\textit{simple motion patterns usually executed by a single person and typically lasting for a very short duration (order of tens of seconds)}''.
Which indicates temporal structure plays an important role in understanding the dynamic in videos and make the task more hard. 
But deep and large 3D CNNS \cite{carreira2017quo,wang2018non,feichtenhofer2019slowfast}, which have attained remarkable success in action recognition, have much more parameters than same structure 2D version. 
Further, learning visual representations generally requires a large number of labeled training example, but manually annotated video are more expensive to collect than image.
Thus, the size and diversity of recently widely-used video datasets (e.g., UCF101, HMDB51, Kinetics) is rather limited (compare to ImageNet). 
Besides, these datasets exist huge implicit bias over scene and object structure \cite{girdhar2019cater,shao2020finegym}, that is, a large amount of samples can be recognized via static object or background. e.g., recognize ``swimming" via water.
All these factors let the base model be easily to overfitting and dwarf variations in temporal structure.

% Thus, obtaining a good video representation without relying on domain specific, annotated samples, has significant impact on real-world scenarios.
Unlabeled video is easy to obtain. 
Self-supervised learning (SSL) aims to pretrain base model with surrogate supervision signal that generate from unlabled data itself, and further transfer the learned model to downstream task.
This topic has been widely studied in the Machine Learning community and achieve highly successful in image-based tasks like image recognition \cite{ye2019unsupervised} and object detection \cite{he2019momentum}.
A key reason for their success is that these methods can be applied on any specific domain and the large size of image dataset.
However, in video-based action recognition, supervised pre-training is still dominant \cite{carreira2017quo,wang2018non}, where self-supervised methods generally lag behind \cite{misra2016shuffle,wang2019self}.
For visual temporal modeling, recent works \cite{misra2016shuffle,lee2017unsupervised} train network to directly learn the embedding under the supervision of \textit{pretext} task, such as the the order of image sequences, puzzle sequence. 
However, these \textit{pretext} tasks has been experimentally shown may be fall into trivial solution \cite{kim2019self} and overfitting to the pre-train objective \cite{yan2019clusterfit}, not generalize to down-stream action recognition.

% =============3.why introduce data augmentation===============
% In contrast to these approaches
These challenges motivate us to study:
how to design an temporal-sensitive, generalize, and efficient video self-supervised framework.
In terms of implicit bias, our intuition is to replace the static background not only don't affect the semantic information but also enrich the diversity of the training dataset.
As shown in Figure \ref{fig:bk_replace}, we can still easily recognize the action ``Tai Chi" as the background replaced.
However, human segmentation for all videos is very time-consuming and not feasible for low-resolution videos.
Instead, we propose novel Temporal Consistent Augmentation (TCA) for video understanding based on this simple observation.
This technique utilizing natural frame from the same or different video as new background, which keep the semantic but large difference in appearance of origin video.
As an data augmentation method, TCA could be applied in a plug-and-play manner to various existing SSL action recognition models to bring consistent improvement.
Besides, the TCA can be implement with simply matrix operation at negligible computation cost.

\input{figures/1-Augment_Background}

% =============4.why introduce VTL===============
Based on TCA, we aim to separate the temporal similarity pairs from dissimilarity pairs in the embedding space on top of the successful contrastive learning \cite{hadsell2006dimensionality}, which good at instance discrimination.
% Action categories naturally have different visual temporal information (e.g. \textit{walk} and \textit{run}).
% When performing the same action, there still exist large variation, due to various factors such as height, age, health. \textit{e.g.}, a professional athlete and a child run at the same time.
Choosing temporal similarity or dissimilarity pairs turns out to be very important for achieving good performance.
Considering video contain both spatial and temporal information, instance discriminative may lay on appearance information under the influence of implicit bias.
Instead, we generate triplets for each video with TCA, and propose a novel video-based triplet loss that inspired by FaceNet \cite{schroff2015facenet}.
To minimize this loss, the network must require strong temporal modeling and not sensitive to implicit bias.
In practical, we propose to do \textit{segment discrimination} instead of \textit{instance discrimination} in video understanding.
This is reasonable because video clips from same video contain similar appearance but large variation in temporal abstraction (e.g. The different steps of the action \textit{archery}).

% =============5.Results & Contribution===============1
Based on our video-based triplet loss, we develop a video-level framework, called Video-based Triplet Learning (VTL) (Figure \ref{fig:teaser}).
Without any bells and whistles, VTL approach/surpass its Imagenet supervised counterpart even better than fully-supervised in thousands level dataset (UCF101 and HMDB51).
In addition, our method also works well on large-scale dataset (Kinetics).
These results show that VTL largely close the gap between unsupervised and supervised representation learning, and can serve as an alternative to ImageNet supervised pre-training in video action recognition.


==> sections/introduction_bk_5_10_2.tex <==
\section{Introduction}
% ======================1.SSL(CL) in image domain===============
Learning visual representations generally requires a large number of labeled training example, but manually annotated data are expensive to collect.
% Thus, obtaining a good video representation without relying on domain specific, annotated samples, has significant impact on real-world scenarios.
Self-supervised learning (SSL) aims to pretrain base model with surrogate supervision signal that generate from data itself, and further transfer the learned model to downstream task.
This topic has been widely studied in the Machine Learning community and achieve highly successful in image-based tasks like image recognition \cite{ye2019unsupervised} and object detection \cite{he2019momentum}.
A key reason for their success is that these methods can be applied on any specific domain and the large size of image dataset.
% especially contrastive learning \cite{hadsell2006dimensionality},

% ======================2.SSL in video domain ()===============
However, in video-based action recognition, supervised pre-training is still dominant \cite{carreira2017quo,wang2018non}, where self-supervised methods generally lag behind \cite{misra2016shuffle,wang2019self}.
Compared with image recognition, the major obstacles lie in that: 
The definition of action is as noted by Turage et al. \cite{turaga2008machine}, ``\textit{simple motion patterns usually executed by a single person and typically lasting for a very short duration (order of tens of seconds)}''.
Which indicates temporal structure plays an important role in understanding the dynamic in videos and make the task more hard. 

However, deep and large 3D CNNS \cite{carreira2017quo,wang2018non,feichtenhofer2019slowfast}, which have attained remarkable success in action recognition, have much more parameters than same structure 2D version. 
% But the size and diversity of recently widely-used video datasets (e.g., UCF101, HMDB51, Kinetics) is rather limited (compare to ImageNet). 
Besides, these datasets exist huge implicit bias over scene and object structure \cite{girdhar2019cater,shao2020finegym}, that is, a large amount of samples can be recognized via static object or background. e.g., recognize ``swimming" via water.
Both two factors let the base model be easily to overfitting and dwarf variations in temporal structure.
% =============3.why introduce data augmentation===============

These challenges motivate us to study:
how to design an temporal-sensitive, effective, and efficient video self-supervised framework with small and bias unlabeled datasets.
% In particular, we build our method on top of the successful 3D CNN architecture which good at tackling the temporal modeling mentioned above.
In terms of limited samples, our intuition is to replace the static background not only don't affect the semantic information but also enrich the diversity of the training dataset.
As shown in Figure \ref{fig:bk_replace}, we can still easily recognize the action ``Tai Chi" as the background replaced.
However, human segmentation for all videos is very time-consuming and not feasible for low-resolution videos.
Instead, we propose novel Temporal Consistent Augmentation (TCA) for video understanding based on this simple observation.
%introducing
This technique utilizing natural frame from the same or different video as new background, which keep the semantic but large difference in appearance of origin video.
As an data augmentation method, TCA could be applied in a plug-and-play manner to various existing SSL action recognition models to bring consistent improvement.
Besides, the TCA can be implement with simply matrix operation at negligible computation cost.

\input{figures/1-Augment_Background}

% =============4.why introduce VTL===============
%why introduce Contrastive Learning
For visual temporal modeling, recent works \cite{misra2016shuffle,lee2017unsupervised} train network to directly learn the embedding under the supervision of \textit{pretext} task, such as the the order of image sequences, puzzle sequence. 
However, these \textit{pretext} tasks has been experimentally shown may be fall into trivial solution \cite{kim2019self} and overfitting to the pre-train objective \cite{yan2019clusterfit}, not generalize to down-stream action recognition.
In contrast to these approaches, we aim to separate the temporal similarity pairs from dissimilarity pairs in the embedding space on top of the successful contrastive learning \cite{hadsell2006dimensionality}, which good at instance discrimination.
% Action categories naturally have different visual temporal information (e.g. \textit{walk} and \textit{run}).
% When performing the same action, there still exist large variation, due to various factors such as height, age, health. \textit{e.g.}, a professional athlete and a child run at the same time.
Choosing temporal similarity or dissimilarity pairs turns out to be very important for achieving good performance.
% In image domain, \cite{ye2019unsupervised,he2019momentum} treat each sample as a instance and the network is trained to tell them apart.
Considering video contain both spatial and temporal information, instance discriminative may lay on appearance information under the influence of implicit bias.
Instead, we generate triplets for each video with TCA, and propose a novel video-based triplet loss that inspired by FaceNet \cite{schroff2015facenet}.
To minimize this loss, the network must require strong temporal modeling and not sensitive to implicit bias.
In practical, we propose to do \textit{segment discrimination} instead of \textit{instance discrimination} in video understanding.
This is reasonable because video clips from same video contain similar appearance but large variation in temporal abstraction (e.g. The different steps of the action \textit{archery}).

% =============5.Results & Contribution===============1

% As our main purpose is to pre-train representations that can be transfered to downstream tasks by fine-tuning. 
% VTL is a mechanism for building dynamic triplet based memory bank for SSL, good at temporal modeling and not sensitive to background. 
Based on our video-based triplet loss, we develop a video-level framework, called Video-based Triplet Learning (VTL) (Figure \ref{fig:teaser}).
Without any bells and whistles, VTL approach/surpass its Imagenet supervised counterpart even better than fully-supervised in thousands level dataset (UCF101 and HMDB51).
In addition, our method also works well on large-scale dataset (Kinetics).
These results show that VTL largely close the gap between unsupervised and supervised representation learning, and can serve as an alternative to ImageNet supervised pre-training in video action recognition.
% The main contributions are:
% \begin{itemize}
%     \item We propose a novel Temporal Consistent Augmentation for video-based self-supervised learning, which reduce the impact of implicit bias and increase diversity of data.
%     \item A novel self-supervised framework that work with any backbones is proposed and achieve significantly improvement in UCF101 and HMDB51.
% \end{itemize}

==> tables/4-1-Backbones.tex <==
\begin{table}
  \caption{Frequency of Special Characters}
  \label{tab:freq}
  \begin{tabular}{ccc}
    \toprule
    Method&HMDB51&UCF101\\
    \midrule
    (2+1)D Scratch & 35.2 & 63.1 \\
    (2+1)D ImageNet & 49.8 & 84.5 \\
    (2+1)D Kinetics & 74.3 & 95.1\\
  \bottomrule
\end{tabular}
\end{table}


==> tables/algorithm.tex <==
%##################################################################################################
\begin{algorithm}[t]
\caption{Pseudocode of PTC in a PyTorch-like style.}
\label{alg:code}
\algcomment{\fontsize{7.2pt}{0em}\selectfont \texttt{bmm}: batch matrix multiplication; \texttt{mm}: matrix multiplication; \texttt{cat}: concatenation.
%\vspace{-1.em}
}
\definecolor{codeblue}{rgb}{0.25,0.5,0.5}
\lstset{
  backgroundcolor=\color{white},
  basicstyle=\fontsize{7.2pt}{7.2pt}\ttfamily\selectfont,
  columns=fullflexible,
  breaklines=true,
  captionpos=b,
  commentstyle=\fontsize{7.2pt}{7.2pt}\color{codeblue},
  keywordstyle=\fontsize{7.2pt}{7.2pt},
%  frame=tb,
}
\begin{lstlisting}[language=python]
# triplet: triplet generation
# f_p: projection networks that mapping feature map into fixed-length vector
# f_q, f_k: encoder networks for query and key
# queue: dictionary as a queue of K keys (CxK)
# m: momentum
# t: temperature

f_k.params = f_q.params  # initialize
for x in loader:  # load a minibatch x with N samples
    # generate triple feature
    a, p, n = triplet(x) # anchor, positive, negative
    a = f_p.forward(f_q.forward(a))  # anchor : NxC
    p = f_p.forward(f_k.forward(p))  # positive: NxC
    n = f_p.forward(f_q.forward(n)) # negative: NxC
    p = p.detach()
    
    # update queue with negative keys
    enqueue(queue, n)
    
    # positive logits: Nx1
    l_pos = bmm(a.view(N,1,C), p.view(N,C,1))
    
    # negative logits: Nx(K)
    l_neg_queue = mm(a.view(N,C), queue.view(C,K))

    # logits: Nx(K+1)
    logits = cat([l_pos, l_neg], dim=1)

    # update queue
    dequeue(queue) # dequeue the earliese minibatch
    
    # contrastive loss
    labels = zeros(N)  # positives are the 0-th
    loss = CrossEntropyLoss(logits/t, labels)
    
    # SGD update: query network
    loss.backward()
    update(f_q.params)

    # momentum update: key network
    f_k.params = m*f_k.params+(1-m)*f_q.params
\end{lstlisting}
\end{algorithm}
%##################################################################################################

==> tables/equation_example.tex <==
\section{Math Equations}


\begin{math}
  \lim_{n\rightarrow \infty}x=0
\end{math},


\begin{equation}
  \lim_{n\rightarrow \infty}x=0
\end{equation}

the \textbf{displaymath}

\begin{displaymath}
  \sum_{i=0}^{\infty} x + 1
\end{displaymath}

\begin{equation}
  \sum_{i=0}^{\infty}x_i=\int_{0}^{\pi+2} f
\end{equation}



